Observation of Anisotropy of TeV Cosmic Rays with Two Years of HAWC

After two years of operation, the High-Altitude Water Cherenkov (HAWC) Observatory has analyzed the TeV cosmic-ray sky over an energy range between $2.0$ and $72.8$ TeV. The HAWC detector is a ground-based air-shower array located at high altitude in the state of Puebla, Mexico. Using 300 light-tight water tanks, it collects the Cherenkov light from the particles of extensive air showers from primary gamma rays and cosmic rays. This detection method allows for uninterrupted observation of the entire overhead sky (2~sr instantaneous, 8.5~sr integrated) in the energy range from a few TeV to hundreds of TeV. Like other detectors in the northern and southern hemisphere, HAWC observes an energy-dependent anisotropy in the arrival direction distribution of cosmic rays. The observed cosmic-ray anisotropy is dominated by a dipole moment with phase $\alpha\approx40^{\circ}$ and amplitude that slowly rises in relative intensity from $8\times10^{-4}$ at 2 TeV to $14\times10^{-4}$ around 30.3 TeV, above which the dipole decreases in strength. A significant large-scale ($>60^{\circ}$ in angular extent) signal is also observed in the quadrupole and octupole moments, and significant small-scale features are also present, with locations and shapes consistent with previous observations. Compared to previous measurements in this energy range, the HAWC cosmic-ray sky maps improve on the energy resolution and fit precision of the anisotropy. These data can be used in an effort to better constrain local cosmic-ray accelerators and the intervening magnetic fields.

==> authors020.tex <==
\author[University of Utah]{A.U.~Abeysekara}


\author[IF-UNAM]{R.~Alfaro}


\author[UNACH]{C.~Alvarez}


\author[UNACH]{R.~Arceo}


\author[UMSNH]{J.C.~Arteaga-Velázquez}


\author[IF-UNAM]{D.~Avila Rojas}


\author[PSU]{H.A.~Ayala Solares}


\author[IF-UNAM]{A.~Becerril}


\author[IF-UNAM]{E.~Belmont-Moreno}


\author[Rochester]{S.Y.~BenZvi}


\author[IA-UNAM]{A.~Bernal}


\author[UW-Madison]{J.~Braun}


\author[UNACH]{K.S.~Caballero-Mora}


\author[INAOE]{T.~Capistrán}


\author[INAOE]{A.~Carramiñana}


\author[IFJ-PAN]{S.~Casanova}


\author[UMSNH]{M.~Castillo}


\author[UMSNH]{U.~Cotti}


\author[FCFM-BUAP]{J.~Cotzomi}


\author[FCFM-BUAP]{C.~De León}


\author[UdG]{E.~De la Fuente}


\author[INAOE]{R.~Diaz Hernandez}


\author[IA-UNAM]{S.~Dichiara}


\author[LANL]{B.L.~Dingus}


\author[UW-Madison]{M.A.~DuVernois}


\author[UdG]{J.C.~Díaz-Vélez}


\author[UMD]{K.~Engel}


\author[UMD]{D.W.~Fiorino}


\author[IA-UNAM]{N.~Fraija}


\author[IF-UNAM]{J.A.~García-González}


\author[IA-UNAM]{F.~Garfias}


\author[IF-UNAM]{A.~González Muñoz}


\author[IA-UNAM]{M.M.~González}


\author[UMD]{J.A.~Goodman}


\author[UW-Madison]{Z.~Hampel-Arias}


\author[ULB]{Z.~Hampel-Arias}


\author[LANL]{J.P.~Harding}


\author[IF-UNAM]{S.~Hernandez}


\author[MTU]{B.~Hona}


\author[UNACH]{F.~Hueyotl-Zahuantitla}


\author[MSFC]{C.M.~Hui}


\author[MTU]{P.~Hüntemeyer}


\author[IA-UNAM]{A.~Iriarte}


\author[MPIK]{A.~Jardin-Blicq}


\author[MPIK]{V.~Joshi}


\author[UNACH]{S.~Kaufmann}


\author[IGeof-UNAM]{A.~Lara}


\author[UNM]{R.J.~Lauer}


\author[IA-UNAM]{W.H.~Lee}


\author[IF-UNAM]{H.~León Vargas}


\author[INAOE]{A.L.~Longinotti}


\author[UPP]{G.~Luis-Raya}


\author[CIC-IPN]{R.~Luna-García}


\author[INFN Padova]{R.~López-Coto}


\author[MPIK]{R.~López-Coto}


\author[PSU]{K.~Malone}


\author[MSU]{S.S.~Marinelli}


\author[FCFM-BUAP]{O.~Martinez}


\author[UMD]{I.~Martinez-Castellanos}


\author[CIC-IPN]{J.~Martínez-Castro}


\author[CINVESTAV]{H.~Martínez-Huerta}


\author[UNM]{J.A.~Matthews}


\author[UAEH]{P.~Miranda-Romagnoli}


\author[FCFM-BUAP]{E.~Moreno}


\author[PSU]{M.~Mostafá}


\author[IFJ-PAN]{A.~Nayerhoda}


\author[ICN-UNAM]{L.~Nellen}


\author[University of Utah]{M.~Newbold}


\author[Rochester]{M.U.~Nisa}


\author[UAEH]{R.~Noriega-Papaqui}


\author[CIC-IPN]{R.~Pelayo}


\author[PSU]{J.~Pretz}


\author[UPP]{E.G.~Pérez-Pérez}


\author[UNM]{Z.~Ren}


\author[Rochester]{C.D.~Rho}


\author[UMD]{C.~Rivière}


\author[INAOE]{D.~Rosa-González}


\author[PSU]{M.~Rosenberg}


\author[MPIK]{E.~Ruiz-Velasco}


\author[IFJ-PAN]{F.~Salesa Greus}


\author[IF-UNAM]{A.~Sandoval}


\author[UC Santa Cruz]{M.~Schneider}


\author[MPIK]{H.~Schoorlemmer}


\author[PSU]{M.~Seglar Arroyo}


\author[LANL]{G.~Sinnis}


\author[UMD]{A.J.~Smith}


\author[University of Utah]{R.W.~Springer}


\author[MPIK]{P.~Surajbali}


\author[GA Tech]{I.~Taboada}


\author[UNACH]{O.~Tibolla}


\author[MSU]{K.~Tollefson}


\author[INAOE]{I.~Torres}


\author[Stanford]{G.~Vianello}


\author[FCFM-BUAP]{L.~Villaseñor}


\author[UW-Madison]{T.~Weisgarber}


\author[MPIK]{F.~Werner}


\author[UW-Madison]{S.~Westerhoff}


\author[UW-Madison]{J.~Wood}


\author[Rochester]{T.~Yapici}


\author[CINVESTAV]{A.~Zepeda}


\author[LANL]{H.~Zhou}


\author[UMSNH]{J.D.~Álvarez}


\address[University of Utah]{Department of Physics and Astronomy, University of Utah, Salt Lake City, UT, USA }

\address[IF-UNAM]{Instituto de F\'{i}sica, Universidad Nacional Autónoma de México, Ciudad de Mexico, Mexico }

\address[UNACH]{Universidad Autónoma de Chiapas, Tuxtla Gutiérrez, Chiapas, México}

\address[UMSNH]{Universidad Michoacana de San Nicolás de Hidalgo, Morelia, Mexico }

\address[PSU]{Department of Physics, Pennsylvania State University, University Park, PA, USA }

\address[Rochester]{Department of Physics \& Astronomy, University of Rochester, Rochester, NY , USA }

\address[IA-UNAM]{Instituto de Astronom\'{i}a, Universidad Nacional Autónoma de México, Ciudad de Mexico, Mexico }

\address[UW-Madison]{Department of Physics, University of Wisconsin-Madison, Madison, WI, USA }

\address[INAOE]{Instituto Nacional de Astrof\'{i}sica, Óptica y Electrónica, Puebla, Mexico }

\address[IFJ-PAN]{Institute of Nuclear Physics Polish Academy of Sciences, PL-31342 IFJ-PAN, Krakow, Poland }

\address[FCFM-BUAP]{Facultad de Ciencias F\'{i}sico Matemáticas, Benemérita Universidad Autónoma de Puebla, Puebla, Mexico }

\address[UdG]{Departamento de F\'{i}sica, Centro Universitario de Ciencias Exactase Ingenierias, Universidad de Guadalajara, Guadalajara, Mexico }

\address[LANL]{Physics Division, Los Alamos National Laboratory, Los Alamos, NM, USA }

\address[UMD]{Department of Physics, University of Maryland, College Park, MD, USA }

\address[MTU]{Department of Physics, Michigan Technological University, Houghton, MI, USA }

\address[MSFC]{NASA Marshall Space Flight Center, Astrophysics Office, Huntsville, AL 35812, USA}

\address[MPIK]{Max-Planck Institute for Nuclear Physics, 69117 Heidelberg, Germany}

\address[IGeof-UNAM]{Instituto de Geof\'{i}sica, Universidad Nacional Autónoma de México, Ciudad de Mexico, Mexico }

\address[UNM]{Dept of Physics and Astronomy, University of New Mexico, Albuquerque, NM, USA }

\address[UPP]{Universidad Politecnica de Pachuca, Pachuca, Hgo, Mexico }

\address[CIC-IPN]{Centro de Investigaci\'on en Computaci\'on, Instituto Polit\'ecnico Nacional, M\'exico City, M\'exico.}

\address[INFN Padova]{INFN and Universita di Padova, via Marzolo 8, I-35131,Padova,Italy}

\address[MSU]{Department of Physics and Astronomy, Michigan State University, East Lansing, MI, USA }

\address[CINVESTAV]{Physics Department, Centro de Investigacion y de Estudios Avanzados del IPN, Mexico City, DF, Mexico }

\address[UAEH]{Universidad Autónoma del Estado de Hidalgo, Pachuca, Mexico }

\address[ICN-UNAM]{Instituto de Ciencias Nucleares, Universidad Nacional Autónoma de Mexico, Ciudad de Mexico, Mexico }

\address[UC Santa Cruz]{Santa Cruz Institute for Particle Physics, University of California, Santa Cruz, Santa Cruz, CA, USA }

\address[GA Tech]{School of Physics and Center for Relativistic Astrophysics - Georgia Institute of Technology, Atlanta, GA, USA 30332 }

\address[Stanford]{Department of Physics, Stanford University: Stanford, CA 94305–4060, USA}

\address[ULB]{Inter-university Institute for High Energies, Universit\'{e} Libre de Bruxelles, Bruxelles, Belgium }


 

